Oblique Decision Trees from Derivatives of ReLU Networks

We show how neural models can be used to realize piece-wise constant functions such as decision trees. The proposed architecture, which we call locally constant networks, builds on ReLU networks that are piece-wise linear and hence their associated gradients with respect to the inputs are locally constant. We formally establish the equivalence between the classes of locally constant networks and decision trees. Moreover, we highlight several advantageous properties of locally constant networks, including how they realize decision trees with parameter sharing across branching / leaves. Indeed, only $M$ neurons suffice to implicitly model an oblique decision tree with $2^M$ leaf nodes. The neural representation also enables us to adopt many tools developed for deep networks (e.g., DropConnect (Wan et al., 2013)) while implicitly training decision trees. We demonstrate that our method outperforms alternative techniques for training oblique decision trees in the context of molecular property classification and regression tasks.

==> src/method-learning.tex <==
\subsection{Learning and computation}\label{sec:learning}
\vspace{-1mm}
In this section, we discuss training algorithms and efficient computation for the proposed models.
% \subsubsection{adfa}

\textbf{Training \textsc{Lcn} and \textsc{Alcn}.} Even though \textsc{Lcn} is sub-differentiable, the network does not exhibit useful gradient information for learning each locally constant representation $\nabla_\vx \va^i_1$ (note that $\vec{J}_\vx \tilde \va^M = [\nabla_\vx \va^1_1,\dots,\nabla_\vx \va^M_1]$) whenever $\vo^i_1 = 0$, since, operationally, $\vo^i_1 = 0$ implies $\va^i_1 \gets 0$ and there is no useful gradient of $\nabla_\vx \va^i_1 = \nabla_\vx 0 = \vzero$ with respect to model parameters. To alleviate the problem, we propose to leverage softplus as an infinitely differentiable approximation of ReLU to obtain meaningful learning signals for $\nabla_\vx \va^i_1$. Concretely, we conduct the annealing during training:
\begin{align}
\vspace{-2mm}
    \va^i_1 = \lambda_t \max(0, \vz^i_1) + (1-\lambda_t) \log (1 + \exp(\vz^i_1)), \forall i \in [M], \lambda_t \in [0, 1], \label{eq:annealing}
\vspace{-2mm}
\end{align}
where $\lambda_t$ is an iteration-dependent annealing parameter. Both \textsc{Lcn} and \textsc{Alcn} can be constructed as a special case of Eq.~(\ref{eq:annealing}). We train \textsc{Lcn} with $\lambda_t$ equal to the ratio between the current epoch and the total epochs, and \textsc{Alcn} with $\lambda_t = 0$. Both models are optimized via gradient descent. 

We also include DropConnect~\citep{wan2013regularization} to the weight matrices $\mW^i \gets \text{drop}(\mW^i)$ during training. Despite the simple structure of DropConnect in the locally constant networks, it entails a structural dropout on the weights in the corresponding oblique decision trees (see \xref{sec:inductive-bias}), which is challenging to reproduce in typical oblique decision trees. In addition, it also encourages the exploration of parameter space, which is easy to see for the raw \textsc{Lcn}: the randomization enables the exploration that flips $\vo^i_1 = 0$ to $\vo^i_1 = 1$ to establish effective learning signal. Note that the standard DropOut~\citep{srivastava2014dropout} is not ideal for the low capacity models that we consider here. 

\textbf{Training \textsc{Elcn}.} Since each ensemble component is sub-differentiable, we can directly learn the whole ensemble through gradient descent. However, the approach is not scalable due to memory constraints in practice. Instead, we propose to train the ensemble in a boosting fashion:
\begin{enumerate}
\vspace{-3mm}
    \item We first train an initial locally constant network $g^{[1]}_{\phi}(\vec{J}_\vx \tilde \va^{M, [1]})$.
\vspace{-2mm}
    \item For each iteration $e' \in \{2,3,\dots,E\}$, we incrementally optimize $\sum_{e=1}^{e'} g^{[e]}_{\phi}(\vec{J}_\vx \tilde \va^{M, [e]})$.
\vspace{-3mm}
\end{enumerate}
Note that, in the second step, only the latest model is optimized, and thus we can simply store the predictions of the preceding models without loading them into the memory. Each partial ensemble can be directly learned through gradient descent, without resorting to complex meta-algorithms such as adaptive boosting~\citep{freund1997decision} or gradient boosting~\citep{friedman2001greedy}. 

\textbf{Computation \camera{and time complexity}.}
\textsc{Lcn} and \textsc{Alcn} are built on the gradients of all the neurons $\vec{J}_\vx \tilde \va^M = [\nabla_\vx \va^M_1,\dots,$ $\nabla_\vx \va^1_1]$, which can be computationally challenging to obtain. Existing automatic differentiation (e.g., back-propagation) only computes the gradient of a scalar output. Instead, here we propose an efficient dynamic programming procedure which only requires a forward pass:
\begin{enumerate}
\vspace{-2mm}
    \item $\nabla_\vx \va^1_1 = \vo^1_1 \times \mW^1$.
    % \item $\nabla_\vx \va^1_1 = {\partial \va^1_1}/{\partial \vz^1_1} \times \mW^1$.
\vspace{-1mm}
    \item $\forall i \in \{2,\dots,M\}, \nabla_\vx \va^i_1 = \vo^i_1 \times (\mW^i_{1, 1:D} + \sum_{k=1}^{i-1} \mW^i_{1, D+k} \nabla_\vx \va^k_1)$,
\vspace{-2.5mm}
\end{enumerate}
% where $\nabla_\vx \va^k_1$ is the computed gradient in the preceding layers. The dynamic programming costs $M + \sum_{i=2}^M (i-1) = O(M^2)$ multiplication and $\sum_{i=2}^M (i-1) = O(M^2)$ addition. Straightforward back-propagation re-computes the partial solutions $\nabla_\vx \va^k_1$ for each $\nabla_\vx \va^i_1$, so the complexity is $O(M^3)$.\!\!\!\!
The complexity of the dynamic programming is $\gO(M^2)$ due to the inner-summation inside each iteration. Straightforward back-propagation re-computes the partial solutions $\nabla_\vx \va^k_1$ for each $\nabla_\vx \va^i_1$, so the complexity is $\gO(M^3)$. We can parallelize the inner-summation on a GPU, and the complexity of the dynamic programming and straightforward back-propagation will become $\gO(M)$ and $\gO(M^2)$, respectively. Note that the complexity of a forward pass of a typical network is also $\gO(M)$ on a GPU. \camera{The time complexity of learning \textsc{Lcn} by gradient descent is thus $\gO(M \tau)$ with some iteration number $\tau$. In contrast, the computation of existing oblique decision tree training algorithm is typically data-dependent and thus the worst-case analysis is not fairly representative.} 

\camera{\textbf{Space complexity.} The space complexity of \textsc{Lcn} is $\gO(MD)$ for realizing decision nodes and $\gO(MDL)$ (assuming a linear $g_\phi$) for realizing leaf nodes. In contrast, the space complexity of oblique decision trees is $\gO((2^M - 1) D)$ for decision nodes and $\gO(2^M L)$ for leaf nodes. Hence, our representation improvements the space complexity exponentially.}

==> src/method-representation.tex <==


\subsection{Representation theory}

In this section, we prove the equivalence between the class of oblique decision trees and the class of locally constant networks. 
We first make an observations:
\begin{itemize}
\vspace{-2mm}
    \item Any network $f_\theta$ can be re-written to have $1$ neuron per layer, by expanding any layer with $N_i > 1$ neurons to be $N_i$ different layers such that they do not have inter-connections. 
    \item Any unbalanced decision tree can be re-written to be balanced by adding dummy decision nodes $\vzero^\top\vx \geq -1$. 
\vspace{-2mm}
\end{itemize}
We define the \emph{class} of locally constant networks with the $1$ constraint:
\begin{definition}
The class of locally constant networks contains any functions that can be written as $g_{\theta'}(\tilde \vo^M)$, where $\tilde \vo^M$ is defined via Eq.~(\ref{eq:forward}-\ref{eq:actpattern}) with $N_i = 1, \forall i \in [M]$ and $M \in \sZ_{\geq 0}$ and $g_{\theta'}: \{0, 1\}^M \to \sR^L$ is a table. 
\end{definition}
And we define the \emph{class} of oblique decision trees with the balance constraint:
\begin{definition}
The class of oblique decision trees contains any functions that can be procedurally defined (with some depth $d \in \sZ_{>0}$) for $\vx \in \sR^D$:
\begin{enumerate}
\vspace{-2mm}
    \item $\vr_1 \triangleq \one [ \hat \vw_{\varnothing}^\top \vx + \hat b_{\varnothing} \geq 0]$, where $\hat \vw_{\varnothing} \in \sR^D$ and $b_\varnothing \in \sR$ denote the weight and bias of the root decision node and $\one [\cdot]$ is the indicator function.
\vspace{-1.5mm}
    \item For $i \in (2,\dots,d), \vr_i \triangleq \one [ \hat \vw_{\vr_{1:i-1}}^\top \vx + \hat b_{\vr_{1:i-1}} \geq 0]$, where $\hat \vw_{\vr_{1:i-1}} \in \sR^D$ and $\hat b_{\vr_{1:i-1}} \in \sR$ denote the weight and bias for the decision node after the decision pattern $\vr_{1:i-1}$.
\vspace{-1.5mm}
    \item $v: \{0, 1\}^d \to \sR^L$ is the leaf output function $v(\vr_{1:d})$ for the decision pattern $\vr_{1:d}$.
\vspace{-2mm}
\end{enumerate}
\end{definition}
We first prove that the class of locally constant networks is a subset of oblique decision trees. 
\begin{theorem}
The class of locally constant networks $\subseteq$ the class of oblique decision trees. 
\end{theorem}
\begin{proof}
For any locally constant networks with $M \in \sZ_{\geq 0}$, we define the following oblique decision tree with $d=M$ for $\vx \in \sR^D$:
\begin{enumerate}
\vspace{-2mm}
    \item $\vr_1 \triangleq \vo^1_1 = \one [ \hat \vw_{\varnothing}^\top \vx + \hat b_{\varnothing} \geq 0]$ with $\hat \vw_{\varnothing} = W^1_{1,:}$ and $b_\varnothing = \vb^1_1$.\!\!\!\!
\vspace{-1mm}
    \item For $i \in (2,\dots,M), \vr_i \triangleq \vo^i_1 = \one [ \hat \vw_{\vr_{1:i-1}}^\top \vx + \hat b_{\vr_{1:i-1}} \geq 0]$, where $\hat \vw_{\vr_{1:i-1}} = \nabla_\vx \vz^i_1$ and $\hat b_{\vr_{1:i-1}} = \vz^i_1 - \vx^\top \nabla_\vx \vz^i_1$.
\vspace{-1mm}
    \item $v = g_{\theta'}$.
\vspace{-2mm}
\end{enumerate}
Note that, in order to be a valid decision tree, $\hat \vw_{1:\vr_{i-1}}$ and $\hat b_{1:\vr_{i-1}}$ have to be unique for all $\vx$ that yield the same decision pattern $\vr_{1:i-1}$. To see this, as $\vr_{1:i-1} = (\vo^1_1,\dots,\vo^{i-1}_1)$, we know the neuron $\vz^i_1$ is a fixed affine function given a fixed activation pattern for all the preceding neurons, so $\nabla_\vx \vz^i_1$ and $\vz^i_1 - \vx^\top \nabla_\vx \vz^i_1$ are fixed quantities given a fixed decision pattern $\vr_{1:i-1}$. As we have $\vr_{1:M} = \tilde \vo^M$ and $v = g_{\theta'}$, we conclude that they yield the same mapping. 
\end{proof}
% We first prove that the class of locally constant networks is a subset of oblique decision trees. 
The other direction is 
\begin{theorem}
The class of locally constant networks $\subseteq$ the class of oblique decision trees. 
\end{theorem}

And we define the \emph{class} of oblique decision trees with the balance constraint:
\begin{definition}
The class of oblique decision trees contains any functions that can be written as $v_{\phi'}(r(\hat \mW \vx + \hat \vb))$, where 
\begin{itemize}
\vspace{-2mm}
    \item $\hat \mW \in \sR^{2^d-1 \times D}$ and $\hat \vb \in \sR^{2^d-1}$ are all the weights and biases in the tree with depth $d$.
\vspace{-1mm}
    \item $r: \sR^{2^d-1} \to [2^d]$ is a function that routes the input to a leaf node. Specifically, $r(\hat \mW \vx + \hat \vb) = l$ for $l \in [2^d]$ iff  
\vspace{-2mm}
\end{itemize}
$\hat \mW \in \sR^{2^d-1 \times D}$ and $\hat \vb \in \sR^{2^d-1}$ are all the weights and biases in the tree with depth $d$

% $\tilde \vo^M$ is defined via Eq.~(\ref{eq:forward}-\ref{eq:actpattern}) with $N_i = 1, \forall i \in [M]$ and $M \in \sZ_{\geq 0}$ and $g_{\theta'}: \{0, 1\}^M \to \sR^L$ is a table. 
\end{definition}


(defined via Eq.~(\ref{eq:forward}-\ref{eq:actpattern})) with any $M \in \sZ_{>0}$ and $N_i \in \sZ_{>0}, \forall i \in [M]$. 
For the class of oblique decision trees, we first make an obervation that 

Assuming that the decision tree has $L$ leaf nodes, $t_\Phi(\vx)$ can be written as
\begin{align}
    t_\Phi(\vx) = v_{\phi_2}(s_{\phi_1}(\vx)), \forall \vx \in \sR^D,
\end{align}
where $s_{\phi_1}: \sR^D \to [L]$ is the \emph{split} function that transform $\vx$ to the index of leaf nodes, and $v_{\phi_2}: [L] \to \sR^C$ is the \emph{value} function that transform the index of leaf nodes to a real vector. 

% For each $l \in [L]$, the tree function is associated with a series of coordinate-wise split for some coordinate $\vx_\idx$ and threshold $\tau$. To simplify presentation, we sort the splits in the order of the left splits $\vx_\idx < \tau$ and then the right splits $\vx_\idx \geq \tau$, and we denote the number of left and right splits as $n_l$ and $(m_l-n_l)$, respectively,  for each $l \in [L]$. The corresponding threshold and index of a split $r \in [m_l]$ are denoted as $\tau_{l, r}$ and $\idx_{l, r}$, respectively. 

Specifically, $s_{\phi_1}(\vx) = l \in [L]$ if 
% \begin{align}
%     \Upsilon_{\phi_1, l}(\vx) := \prod_{r \in [n_l]} \sI(\vx_{\idx_{l,r}} < \tau_{l,r} ) \prod_{r \in [m_l]\backslash[n_l]} \sI(\vx_{\idx_{l,r}} \geq \tau_{l,r} ) = 1.
% \end{align}
Note that, $\forall \vx \in \sR^D$, the following equivalence holds for a valid decision tree:
% \begin{itemize}
%     \item $\Upsilon_{\phi_1, l}(\vx) = 1 \iff \frac{1}{m_l} (\sum_{r \in [n_l]} \sI(\vx_{\idx_{l, r}} < \tau_{l, r} )  + \sum_{r \in [m_l]\backslash [n_l]} \sI(\vx_{\idx_{l,r}} \geq \tau_{l,r} )) = 1$.
%     \item $\sum_{l \in [L]} \Upsilon_{\phi_1, l}(\vx) = 1$.
% \end{itemize}


We define the class of oblique decision trees as follows:
\begin{definition}
aadfs
\end{definition}

any binary decision trees, where each internal node is associated with a linear classifier and each leaf node is associated with a real output, with finite depth. Note that we do not have to assume balanced branching for the decision trees, or $1$ neuron per layer for locally constant networks. We have
\begin{theorem}
The class of locally constant networks is equivalent to the class of oblique decision trees. 
\end{theorem}

\begin{proof}

\end{proof}



